Policy Design for Active Sequential Hypothesis Testing using Deep Learning

Information theory has been very successful in obtaining performance limits for various problems such as communication, compression and hypothesis testing. Likewise, stochastic control theory provides a characterization of optimal policies for Partially Observable Markov Decision Processes (POMDPs) using dynamic programming. However, finding optimal policies for these problems is computationally hard in general and thus, heuristic solutions are employed in practice. Deep learning can be used as a tool for designing better heuristics in such problems. In this paper, the problem of active sequential hypothesis testing is considered. The goal is to design a policy that can reliably infer the true hypothesis using as few samples as possible by adaptively selecting appropriate queries. This problem can be modeled as a POMDP and bounds on its value function exist in literature. However, optimal policies have not been identified and various heuristics are used. In this paper, two new heuristics are proposed: one based on deep reinforcement learning and another based on a KL-divergence zero-sum game. These heuristics are compared with state-of-the-art solutions and it is demonstrated using numerical experiments that the proposed heuristics can achieve significantly better performance than existing methods in some scenarios.

==> doc/latex/IEEEconf/README <==
              +---------------------------------------+
              |          THE IEEECONF CLASS           |
              | By Scott Pakin, scott+iecnf@pakin.org |
              +---------------------------------------+

Description
===========

The IEEEconf class implements the formatting dictated by the IEEE
Computer Society Press for conference proceedings
(ftp://pubftp.computer.org/press/outgoing/proceedings/instruct8.5x11.pdf).
IEEEconf.cls replaces latex8.sty and is compatible with any BibTeX
style, not just latex8.bst.  The goal was to produce a more faithful
implementation of the formatting rules and to do so with cleaner LaTeX
code than that provided by the latex8.* files.


Installation
============

Execute "latex IEEEconf.ins" to create IEEEconf.cls.  Install
IEEEconf.cls at an appropriate place in your directory tree (e.g., in
/usr/local/share/texmf/tex/latex/IEEEconf/ or
C:\localtexmf\tex\latex\IEEEconf\) and update the filename database,
if necessary.  See the UK TeX FAQ (http://www.tex.ac.uk/faq) for more
information on installing classes.

IEEEconf comes with prebuilt PDF documentation formatted for
U.S. Letter paper.  If you want to build the documentation from
scratch, the procedure is as follows:

    latex IEEEconf.dtx
    makeindex -s gind.ist IEEEconf
    makeindex -s gglo.ist IEEEconf.glo -o IEEEconf.gls
    latex IEEEconf.dtx


License
=======

Copyright (C) 2009 by Scott Pakin

This file may be distributed and/or modified under the conditions of
the LaTeX Project Public License, either version 1.3c of this license
or (at your option) any later version.  The latest version of this
license is in:

   http://www.latex-project.org/lppl.txt

and version 1.3c or later is part of all distributions of LaTeX
version 2006/05/20 or later.

